Residual Reward Models: Leveraging Prior Knowledge for Efficient Preference-based Reinforcement Learning in Robotics

Preference-based Reinforcement Learning (PbRL) provides a promising alternative to heuristic reward design in complex robotic environments. However, PbRL often suffers from poor sample efficiency, requiring extensive and costly human feedback, which limits its real-world applicability. Prior work has proposed learning a reward model from demonstrations and fine-tuning it using preferences. However, when the model is a neural network, transitioning between different loss functions across training phases often leads to unstable optimization and performance degradation. In this paper, we propose a method to effectively leverage prior knowledge with a Residual Reward Model (RRM). An RRM assumes that the true reward of the environment can be split into a sum of two parts: a prior reward and a learned reward. The prior reward is a term available before training, such as an engineering heuristic ``best guess'', a language-generated reward, or a reward function learned from inverse reinforcement learning, and the learned reward is then trained with preferences as a residual offset. Experimental results in Meta-World and DM-Control show that RRMs substantially improve the sample efficiency of common PbRL methods across various prior reward types. Furthermore, we demonstrate the practical efficacy of our method on a physical Franka Panda robot, accelerating policy learning and achieving high success rates in fewer steps than baselines.

==> preamble.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}


\usepackage{colortbl}
\usepackage{makecell}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{pifont}

%icons
\usepackage{fontawesome}
\usepackage{academicons}
\usepackage{titletoc}


\newcommand*{\cf}{\emph{cf.}\@\xspace}
\newcommand*{\eg}{\emph{e.g.}\@\xspace}
\newcommand*{\etal}{\emph{et~al.}\@\xspace}
\newcommand*{\etc}{\emph{etc.}\@\xspace}
\newcommand*{\ie}{\emph{i.e.}\@\xspace}

\usepackage{tabularx}
\usepackage{booktabs}
\usepackage[table]{xcolor} 


\RequirePackage{algorithm}
\RequirePackage{algpseudocode}
\algtext*{EndIf}
\algtext*{EndFor}
\algtext*{EndWhile}
\algtext*{EndProcedure}

